Catastrophe Insurance: An Adaptive Robust Optimization Approach

The escalating frequency and severity of natural disasters, exacerbated by climate change, underscore the critical role of insurance in facilitating recovery and promoting investments in risk reduction. This work introduces a novel Adaptive Robust Optimization (ARO) framework tailored for the calculation of catastrophe insurance premiums, with a case study applied to the United States National Flood Insurance Program (NFIP). To the best of our knowledge, it is the first time an ARO approach has been applied to for disaster insurance pricing. Our methodology is designed to protect against both historical and emerging risks, the latter predicted by machine learning models, thus directly incorporating amplified risks induced by climate change. Using the US flood insurance data as a case study, optimization models demonstrate effectiveness in covering losses and produce surpluses, with a smooth balance transition through parameter fine-tuning. Among tested optimization models, results show ARO models with conservative parameter values achieving low number of insolvent states with the least insurance premium charged. Overall, optimization frameworks offer versatility and generalizability, making it adaptable to a variety of natural disaster scenarios, such as wildfires, droughts, etc. This work not only advances the field of insurance premium modeling but also serves as a vital tool for policymakers and stakeholders in building resilience to the growing risks of natural catastrophes.

==> refs.tex <==
Catastrophe Modeling traditionally is based on simulations of different scenarios. 

Catastrophes are rare fortunately, but it is exactly their rarity that
makes estimating losses from—and preparing for—future catastrophes so difficult. Standard actuarial techniques are insufficient because of the scarcity of
historical loss data. Furthermore, the usefulness of the loss data that does exist
is limited because the landscape of what is insured is constantly changing. 

Optimization models for catastrophe insurance premium pricing:
- Stochastic Optimization (Ermoliev et al) talks about using stochastic optimization to model insurance portfolios of catastrophe risks. The paper discusses modelling dependencies in order to maximise profit.

- Flood Catastrophe Model (Ermolieva) talks about applying a stochastic optimization model for Flood insurance program specifically in the Netherlands. 


\cite{ch4} discusses the impact of climate change and catastrophe modelling. 


\cite{risk management and climate change} highlights the value of robust decision-making tools for climate policies. 


from ChatGPT: 
Advances in Modeling Techniques: Over the years, there has been a significant advancement in modeling techniques for catastrophe events. Traditional approaches have evolved into more sophisticated and comprehensive models, integrating geospatial data, climate variables, and socioeconomic factors. The use of high-resolution data, remote sensing, and machine learning algorithms has improved the accuracy and precision of catastrophe models.

Uncertainty and Risk Assessment: Researchers have recognized the importance of quantifying uncertainties associated with catastrophe modeling. There is a growing emphasis on uncertainty analysis and probabilistic approaches to assess the range of potential outcomes. This helps in better understanding the inherent uncertainties in model inputs, assumptions, and parameter estimation, leading to more reliable risk assessments.

Integration of Climate Change: Catastrophe modeling has increasingly incorporated the effects of climate change on natural disasters. Researchers are exploring how climate change influences the frequency, intensity, and spatial distribution of events. Incorporating climate projections and considering the uncertainties associated with climate change impacts have become crucial aspects of robust catastrophe models.

==> structure.tex <==
Introduction

Related Works
- Catastrophe Insurance 
- Robust Optimization 

Optimization Framework 
- Deterministic LP formulation 
- RO formulation 
- with ML predictions 

Case study to flood insurance
- Data set 
- Parameter estimation 
- ML model prediction 
- Results 

Conclusion & evaluation 

